Hamiltonian Cycle Construction in Rectangular Grid Graphs with Three-Stacked Triangular Holes

The Hamiltonian cycle problem is NP-complete for general grid graphs, while several structured classes admit efficient construction algorithms. In this paper, we investigate Hamiltonian cycle construction in rectangular grid graphs containing a three-stacked right-triangular hole. We explore two complementary approaches based on the geometric structure of the hole and the parity properties of rectangular subgraphs. The first approach constructs a Hamiltonian path in the complementary reversed staircase region, extends it into an inner Hamiltonian cycle, and merges it with a cycle in the surrounding graph. The second approach partitions the graph into six rectangular subgraphs and constructs a global Hamiltonian cycle by merging local cycles along compatible boundaries. When odd-sized rectangular subgraphs prevent direct cycle construction, we develop parity-based repartitioning techniques that transform selected configurations into even-sized rectangles. We provide constructions for adjacent and nonadjacent odd-sized configurations and investigate reductions for cases involving multiple odd-sized regions. These results establish a constructive framework for Hamiltonian cycles in grid graphs with staircase-shaped holes and identify the remaining cases requiring further analysis.

==> section6-diagrams.tex <==

\begin{figure}[htbp]
\centering
\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{tikzpicture}[scale=0.42]
\fill[orange!22] (0,3) rectangle (7,6);
\fill[orange!35] (0,0) rectangle (3,3);
\draw[thick] (0,0)--(3,0)--(3,3)--(7,3)--(7,6)--(0,6)--cycle;
\draw[very thick,dashed,red!70!black] (0,3)--(3,3);
\node at (3.5,4.5) {$7\times3$};
\node at (1.5,1.5) {$3\times3$};
\end{tikzpicture}
\caption{Two odd rectangles; original horizontal interface.}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{tikzpicture}[scale=0.42]
\fill[blue!18] (0,0) rectangle (3,6);
\fill[green!20] (3,3) rectangle (7,6);
\draw[thick] (0,0)--(3,0)--(3,3)--(7,3)--(7,6)--(0,6)--cycle;
\draw[very thick,blue!70!black] (3,3)--(3,6);
\node at (1.5,3) {$3\times6$};
\node at (5,4.5) {$4\times3$};
\end{tikzpicture}
\caption{New vertical interface; both rectangles are even-sized.}
\end{subfigure}

\medskip
\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{tikzpicture}[scale=0.42]
\fill[orange!22] (0,0) rectangle (3,7);
\fill[orange!35] (3,0) rectangle (6,3);
\draw[thick] (0,0)--(6,0)--(6,3)--(3,3)--(3,7)--(0,7)--cycle;
\draw[very thick,dashed,red!70!black] (3,0)--(3,3);
\node at (1.5,4.5) {$3\times7$};
\node at (4.5,1.5) {$3\times3$};
\end{tikzpicture}
\caption{Two odd rectangles; original vertical interface.}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{tikzpicture}[scale=0.42]
\fill[blue!18] (0,0) rectangle (6,3);
\fill[green!20] (0,3) rectangle (3,7);
\draw[thick] (0,0)--(6,0)--(6,3)--(3,3)--(3,7)--(0,7)--cycle;
\draw[very thick,blue!70!black] (0,3)--(3,3);
\node at (3,1.5) {$6\times3$};
\node at (1.5,5) {$3\times4$};
\end{tikzpicture}
\caption{New horizontal interface; both rectangles are even-sized.}
\end{subfigure}
\caption{Adjacent-pair repartitioning in two orientations. Dimensions
count vertex columns and rows; the blocks represent disjoint vertex
sets, not individual grid cells. Dashed red lines mark the old partition
interfaces, and solid blue lines mark the new ones. The union is unchanged.}
\label{fig:adjacent-odd-repartition}
\end{figure}

\begin{figure}[htbp]
\centering
\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{tikzpicture}[scale=0.78,every node/.style={font=\small}]
\coordinate (A) at (0,2);
\coordinate (B) at (-1.73,1);
\coordinate (C) at (-1.73,-1);
\coordinate (D) at (0,-2);
\coordinate (G_2) at (1.73,-1);
\coordinate (G_1) at (1.73,1);
\draw[black!45] (A)--(B);
\draw[black!45] (B)--(C);
\draw[black!45] (C)--(D);
\draw[black!45] (D)--(G_2);
\draw[black!45] (G_2)--(G_1);
\draw[black!45] (G_1)--(A);
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (A) {$A$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (B) {$B$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (C) {$C$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (D) {$D$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (G_2) {$G_2$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (G_1) {$G_1$};
\end{tikzpicture}
\caption{One intervening rectangle: $A,B,C$.}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{tikzpicture}[scale=0.78,every node/.style={font=\small}]
\coordinate (A) at (0,2);
\coordinate (B) at (-1.73,1);
\coordinate (C) at (-1.73,-1);
\coordinate (D) at (0,-2);
\coordinate (G_2) at (1.73,-1);
\coordinate (G_1) at (1.73,1);
\draw[black!45] (A)--(B);
\draw[black!45] (B)--(C);
\draw[black!45] (C)--(D);
\draw[black!45] (D)--(G_2);
\draw[black!45] (G_2)--(G_1);
\draw[black!45] (G_1)--(A);
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (A) {$A$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (B) {$B$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (C) {$C$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (D) {$D$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (G_2) {$G_2$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (G_1) {$G_1$};
\end{tikzpicture}
\caption{Two intervening rectangles: $A,B,C,D$.}
\end{subfigure}
\caption{The two nonadjacent configurations in the cyclic adjacency
order. Orange nodes denote odd-sized rectangles and white nodes denote
even-sized rectangles. These diagrams describe relative positions only;
they do not yet specify repartitioning constructions.}
\label{fig:nonadjacent-odd-layouts}
\end{figure}

\begin{figure}[htbp]
\centering
\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{tikzpicture}[scale=0.78,every node/.style={font=\small}]
\coordinate (A) at (0,2);
\coordinate (B) at (-1.73,1);
\coordinate (C) at (-1.73,-1);
\coordinate (D) at (0,-2);
\coordinate (G_2) at (1.73,-1);
\coordinate (G_1) at (1.73,1);
\draw[very thick,blue!70!black] (A)--(B);
\draw[black!45] (B)--(C);
\draw[black!45] (C)--(D);
\draw[black!45] (D)--(G_2);
\draw[black!45] (G_2)--(G_1);
\draw[black!45] (G_1)--(A);
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (A) {$A$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (B) {$B$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (C) {$C$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (D) {$D$};
\node[draw,circle,fill=white,minimum size=9mm,inner sep=1pt] at (G_2) {$G_2$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (G_1) {$G_1$};
\end{tikzpicture}
\caption{Four odd rectangles: select the adjacent pair $A,B$.
The remaining odd rectangles are $D,G_1$.}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.47\textwidth}
\centering
\begin{tikzpicture}[scale=0.78,every node/.style={font=\small}]
\coordinate (A) at (0,2);
\coordinate (B) at (-1.73,1);
\coordinate (C) at (-1.73,-1);
\coordinate (D) at (0,-2);
\coordinate (G_2) at (1.73,-1);
\coordinate (G_1) at (1.73,1);
\draw[very thick,blue!70!black] (A)--(B);
\draw[black!45] (B)--(C);
\draw[very thick,blue!70!black] (C)--(D);
\draw[black!45] (D)--(G_2);
\draw[very thick,blue!70!black] (G_2)--(G_1);
\draw[black!45] (G_1)--(A);
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (A) {$A$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (B) {$B$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (C) {$C$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (D) {$D$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (G_2) {$G_2$};
\node[draw,circle,fill=orange!35,minimum size=9mm,inner sep=1pt] at (G_1) {$G_1$};
\end{tikzpicture}
\caption{Six odd rectangles: select the three disjoint pairs
$A,B$; $C,D$; and $G_2,G_1$.}
\end{subfigure}
\caption{Pair selection for the four- and six-odd cases. Orange nodes
are odd-sized rectangles; thick blue edges indicate pairs chosen for
the adjacent-pair repartitioning. The four-odd layout is one example,
not an enumeration of all placements. These diagrams show pair selection,
not the updated interfaces or the final cycle-merging edges.}
\label{fig:four-six-odd-pairs}
\end{figure}

